Effective Heterogeneous Federated Learning via Efficient Hypernetwork-based Weight Generation

While federated learning leverages distributed client resources, it faces challenges due to heterogeneous client capabilities. This necessitates allocating models suited to clients' resources and careful parameter aggregation to accommodate this heterogeneity. We propose HypeMeFed, a novel federated learning framework for supporting client heterogeneity by combining a multi-exit network architecture with hypernetwork-based model weight generation. This approach aligns the feature spaces of heterogeneous model layers and resolves per-layer information disparity during weight aggregation. To practically realize HypeMeFed, we also propose a low-rank factorization approach to minimize computation and memory overhead associated with hypernetworks. Our evaluations on a real-world heterogeneous device testbed indicate that \system enhances accuracy by 5.12% over FedAvg, reduces the hypernetwork memory requirements by 98.22%, and accelerates its operations by 1.86x compared to a naive hypernetwork approach. These results demonstrate HypeMeFed's effectiveness in leveraging and engaging heterogeneous clients for federated learning.

==> sec/temp.tex <==
The recently evolving paradigm of distributed training via federated learning offers a novel approach to developing effective models by utilizing data collected on end devices such as IoT and mobile platforms. This method enables the system to fully exploit data from many clients while maintaining a privacy-aware environment by ensuring that raw data remains on the client's devices.

To fully leverage this distributed data, it is crucial to maximize the number of clients participating in the federated learning process. However, studies highlight that opportunities for participation are often limited due to various factors. A major obstacle is the heterogeneity of computing resources, which can limit both model performance and client participation. It is unrealistic to assume that all clients have similar computing resources and can train the same model. Clients with limited resources (e.g., CPU, RAM, GPU) may be unable to join the training process, despite possessing valuable data. Conversely, if the server employs a lightweight model to accommodate as many clients as possible, the performance of clients with ample resources can be constrained by the limited model capacity. Additionally, less capable clients may require extensive training time, potentially exceeding the server's deadline and preventing their participation.

To accommodate the diverse range of computing resources in clients with heterogeneous capabilities, a server can transmit models with different levels of capacity (i.e., number of parameters) suitable for each client. A model with a relatively small number of parameters generally requires less memory, computation, and latency for both inference and training~\cite{horvath2021fjord}. However, applying this to federated learning presents a challenge: the server must aggregate knowledge from locally trained models with non-identical architectures. One feasible approach is to exploit a subnetwork architecture within the full neural network by splitting the network in a depth-wise manner (e.g., layer-level split). While promising, we identify two notable issues with the naive approach of simply dividing the network in a depth-wise manner.

\noindent \textbf{[Issue 1] Misaligned Feature Space:}
The first issue with depth-wise network splits is the \textit{misaligned feature space}. Layers closer to the input focus on local features, while layers closer to the output capture global features for tasks like classification. When devices with varying capabilities hold different ``splits'' of the network, the feature spaces for the same layer can differ due to their relative positions in subnetworks. For example, a layer might act as an intermediate layer in the full model but as a final layer in a subnetwork. This misalignment can significantly harm model performance in federated learning, as also reported by Luo et al.~\cite{luo2021no}.

\noindent \textbf{[Solution 1] Multi-exit Architecture:}
To better align the representation space in each subnetwork, we leverage a \textit{multi-exit architecture}\cite{teerapittayanon2016branchynet, laskaridis2021adaptive}. This approach enables each depth-wise split subnetwork to independently learn global features while also exploiting them as local features for subsequent subnetworks. By using a multi-exit architecture, we achieve improved feature alignment in models with different layer depths. This ensures that each layer contributes to both local and global feature learning, enhancing the overall performance and consistency of the federated learning process. We will discuss more about the multi-exit architecture and its implementation in Section~\ref{sec:design}.



\noindent \textbf{[Issue 2] Per-layer information disparity:}
Figure~\ref{fig:prelim-ME} visualizes the operations of a naive parameter aggregation scheme at the federated learning server for clients operating heterogeneous models. Unlike the earlier layers (closer to the input, depicted in pink) shared across all subnetworks, the number of gathered parameters for the deeper layers can be limited (green and blue). This occurs because all clients execute the earlier (shallow) layers of the model, but only clients with sufficient resources execute the deeper layers. Consequently, when aggregated at the server, the quantities of gathered weights differ for each network layer, depending on how subnetworks are distributed in the network. We define this \textit{per-layer information disparity} as the second issue in realizing depth-wise network splits in federated learning. This issue, where specific layers in the neural network receive less information to aggregate, hinders proper model convergence and generalization.

\noindent \textbf{[Solution 2] Hypernetwork-based network parameter generation:} To address this issue, we explore leveraging a \textit{hypernetwork for network parameter generation}. Hypernetworks use a set of network parameters to generate the weights for a different network. Figure~\ref{fig:prelim-HN} illustrates how a hypernetwork architecture can be used for federated learning network weight generation. Specifically, the hypernetwork takes the trained parameters from the shallow layers and generates the necessary parameters for deeper layers to facilitate effective aggregation. By doing so, we can generate weights for the $n^{th}$ layer using the $n-1^{th}$ layer weights. This resolves the information disparity issue occurring at the deep layers of heterogeneous federated learning. We emphasize that the hypernetwork is trained on the server using model parameters obtained from clients.





In federated learning, the diversity in device capabilities and data distributions poses significant challenges, particularly in achieving optimal model performance across heterogeneous environments. This paper addresses the issue of information disparity in federated learning by introducing a novel approach that leverages hypernetworks to generate personalized models for each device. To enhance the efficiency and scalability of our approach, we propose a hypernetwork design employing low rank factorization techniques. This design not only reduces computational overhead but also maintains high accuracy and adaptability to varying device contexts. Our experimental results demonstrate that the proposed method significantly outperforms traditional FL models in terms of both accuracy and computational efficiency, making it a promising solution for real-world heterogeneous federated learning applications. By bridging the gap between model personalization and resource constraints, this work lays a foundation for more inclusive and effective federated learning systems.



A multi-exit architecture is widely employed in deep neural networks to enhance inference latency by enabling adaptive inference and eliminating unnecessary operations~\cite{}. Teerapittayanon et al. introduced BranchNet, a pioneering multi-exit deep neural network featuring multiple classifiers integrated within the baseline model to achieve adaptive inference and improve computational latency~\cite{teerapittayanon2016branchynet}. Given that mobile and embedded devices often experience lagging inference, multi-exit architectures are extensively applied in various real-world sensing applications within mobile and embedded computing environments~\cite{}.



Hypernetworks, originally introduced by Ha et al. \cite{ha2016hypernetworks}, are neural networks designed to generate weights for another neural network, offering flexibility and adaptability in various applications such as computer vision \cite{jia2016dynamic, klocek2019hypernetwork} and 3D scene representation \cite{littwin2019deep, sitzmann2020implicit}. In the context of federated learning, Shamsian et al. proposed pFedHN \cite{shamsian2021personalized}, which employs hypernetworks trained in a federated manner to enhance model initialization and personalization. Ma et al. \cite{ma2022layer} utilized hypernetworks to determine aggregation ratios between models, thereby improving personalized models for individual clients. However, existing efforts primarily focus on hypernetwork training or model personalization within federated learning frameworks.

To our knowledge, \system represents a novel approach in the field by leveraging hypernetworks specifically to address challenges posed by heterogeneous federated learning scenarios. Unlike previous works that either train hypernetworks for general model initialization or focus on personalizing models, our approach aims to generate missing model parameters dynamically, accommodating varying computational resources among federated clients. This innovative use of hypernetworks in \system facilitates effective model aggregation and adaptation across diverse client devices, thereby enhancing both model performance and convergence in federated learning settings.










While a majority of federated learning research has focused on homogeneous model architectures with little consideration on the clients' computing capabilities, supporting heterogeneous federated learning is crucial as it allows for tailored models that can adapt to the diverse computational capabilities, data distributions, and privacy requirements of different devices within the network. Unlike a uniform model approach, heterogeneous federated learning enhances the overall system's efficiency and accuracy by leveraging the unique strengths of each device, ensuring that even resource-constrained devices can contribute effectively. This inclusivity not only improves the robustness and personalization of the models but also maximizes the potential of the collective data, leading to better generalization and performance across various tasks and environments.

Recent works have aimed to accommodate clients with heterogeneous computational resources for federated learning in real-world mobile/embedded applications. One of the initial approaches relied primarily on (i) knowledge distillation (KD)~\cite{hinton2015distilling} to share the knowledge embedded in models with heterogeneous architectures~\cite{}. Li and Wang proposed FedMD~\cite{li2019fedmd}, which transmits a proxy dataset (i.e., the probability distribution of the training dataset) instead of model parameters. Each client then runs an additional distillation process to achieve consensus among the models. Similarly, Seo et al.~\cite{seo202216} proposed federated knowledge distillation to enable heterogeneous federated learning. However, these methods assume the availability of shared public datasets on either the server or local users, limiting system scalability. Additionally, FedMD introduces extra computational costs, posing constraints in federated learning for mobile/embedded computing scenarios.

Another approach is to exploit (ii) shared submodel architectures. HeteroFL~\cite{diao2020heterofl} leverages different ratios of a given full model's parameters to accommodate heterogeneous client models. ScaleFL~\cite{ilhan2023scalefl} employs a strategy of splitting the model in both depth and width, combined with knowledge distillation. However, such approaches suffer from information imbalance problems in relatively large capacity models~\cite{yao2021fedhm}.

A further potential approach is to use (iii) model pruning techniques, which apply masks to reduce model capacity. FedRolex~\cite{alam2022fedrolex} introduced a rolling submodel extraction method to support dynamic model capacity. LotteryFL~\cite{li2020lotteryfl} and Hermes~\cite{li2021hermes} applied a shared pruning mask to adjust model capacity.




























































Now we present a preliminary study to demonstrate the aforementioned challenges and the feasibility of the proposed system.

We used the FashionMNIST dataset independently and identically distributed across a total of 50 clients and 10 randomly selected clients participating in the federated learning process each round.
Specifically, we conduct the experiments in three different model architectures with respect to the model depth.
We designed the full model with three convolution layers and considered scenarios where 17, 17, and 16 clients can afford 1, 2, and 3 layered models, respectively, during the training process.
As a practically possible scenario, we used two baselines: one where all clients use the single-layered model and another where only clients capable of utilizing the three-layered model participate in the training process.

Figure~\ref{fig:prelim} (c) shows the accuracy trend across different settings.
Unsurprisingly, the deeper model showed higher performance compared to the lighter model with a single layer.
However, in the federated learning scenario with only a limited number of participants who can exploit the large model, the deeper model failed to achieve superior performance, even performing worse than the scenario where all clients used the lightest model.
This highlights the need for an advanced approach to fully utilize the data from both the perspectives of participation opportunity and model capacity.
Here, we demonstrate the effectiveness of the proposed multi-exit architecture and hypernetwork, allowing all clients to participate with an appropriate capacity model.
In the absence of the multi-exit architecture, we observe that convergence fails due to the issue of misaligned feature space (see Sec~\ref{subsec:3.1}).
Similarly, without the hypernetwork, convergence fails due to the issue of per-layer information disparity establishing the need for both multi-exit and hypernetwork approaches.

To better convey the operational principles of the proposed scheme, we conducted further analysis.
First, we measured the feature space similarity to confirm the issue of misaligned feature space.
Figure~\ref{fig:prelim2} (a) depicts the similarity of representation spaces in each client, measured by Centered Kernel Alignment (CKA)~\cite{} which is a similarity measure designed to measure the similarity of features from neural networks.

The naive approach showed that models learned relatively different features (CKA=0.8) despite having identical architectures, leading to convergence issues.
When the multi-exit architecture is applied, it demonstrates improved feature alignment (CKA=0.85), consolidating the need to exploit multi-exit architecture in depth-wise split networks in federated learning scenarios.
This demonstrates the feasibility of the proposed approach.


